One-shot World Models Using a Transformer Trained on a Synthetic Prior

A World Model is a compressed spatial and temporal representation of a real world environment that allows one to train an agent or execute planning methods. However, world models are typically trained on observations from the real world environment, and they usually do not enable learning policies for other real environments. We propose One-Shot World Model (OSWM), a transformer world model that is learned in an in-context learning fashion from purely synthetic data sampled from a prior distribution. Our prior is composed of multiple randomly initialized neural networks, where each network models the dynamics of each state and reward dimension of a desired target environment. We adopt the supervised learning procedure of Prior-Fitted Networks by masking next-state and reward at random context positions and query OSWM to make probabilistic predictions based on the remaining transition context. During inference time, OSWM is able to quickly adapt to the dynamics of a simple grid world, as well as the CartPole gym and a custom control environment by providing 1k transition steps as context and is then able to successfully train environment-solving agent policies. However, transferring to more complex environments remains a challenge, currently. Despite these limitations, we see this work as an important stepping-stone in the pursuit of learning world models purely from synthetic data.

==> 4_experiments_old.tex <==
\section{Experiments}

% compute cascadelake: from now until next week: 1x128
% last 3 weeks: 2x64

\subsection{One synthetic prior to cover multiple environments}
In this section we would show that the One-shot World Model is able mimic the dynamics of multiple different grid world environments.
Using just 1000 steps as context, we are able to train an agent solving the environemnt on the one-shot world model.

%In the first set of experiments we seek to show that our OSWM can provide, world dynamics and rewards for multiple different environments solely by receiving 1000 steps of context.
%- Use synthetically trained OSWM and show agents can be trained on different grid world
%- Use agent performance vs. agent trained on grid world itself

% super simple environment: grid world
% sample differently sized grid worlds
% idea: empirical motivation / transfer to multiple environments seems to work

\subsection{Increase Environment Complexity}
Here we would show that the same OSWM as before, is capable to extend to more complex environments, namely CartPole and Acrobot.
Both having continuous states and discrete actions.
We show learning curve of the agent on the OSWN (such as Fig. \ref{fig:cartpole-placeholder} TODO over multiple seeds) and provide relative performance compared to a agent trained on the environment itself. 
Another baseline can be the performance of an agent trained using only 1000 steps or the number of steps to achieve same performance as agent trained on One-shot world model.

% To Show the capabilities to scale to more complex environments beyond grid worlds, we show that our OSWM is able to train an agent for the CartPole environment.

\begin{figure}
    \centering
    \includegraphics[width=75mm]{img/PlaceholderCartPoletrainedonOSWM.png}
    \caption{Learning Curve of Agent on OSWM conditioned on Cartpole context. With training episodes on the x-axis and cummulative episode reward on the y axis. Blue shows the training episode reward on OSWM, with its 10 episode running mean in green. Orange is the average test reward on the real environment over 10 test episodes, calculated after each training episode, with the 10 episode running mean in red.}
    \label{fig:cartpole-placeholder}
\end{figure}

%- report results for training agent on OSWM for CartPole, relative performance to trained on real env, number of real steps needed compared to real agent
% idea: OSWM covers multiple environments: show cartpole and acrobot
% changing dimensionalities between envs
% discrete environments work well; potentially continuous as well

\subsection{Continuous Action Space Environments}
Here the One-shot world model is extended to continuous action spaces. 
Where we show the ability to train an agent to solve the environments.
This is first shown using a simple toy environment, with 1-D state and 1-D action, where the ideal action is inverse of the current state.
Afterwards this is extended to gym environments with continuous actions. 
Where Pendulum is the simpler variant with lower state and action dimensionality and reacher with two dimensional actions and higher dimensional states.


\subsection{Context matters}
%The predictive performance of the OSWM is influenced by the context it is provided with.
%Ideally the context provides good coverage of the environment, which concerns both contents and size.
%For this reason we compare different sizes of context and methods to generate it.
Here we look at how the context influences the performance of the One-shot world model.
First we compare different sizes contexts. 
Then how the context is gathered. We look at cheap readily available methods of gathering context, namely random actions, random actions with repeats and temporal epsilon greedy exploration.

%- compare validation accuracy for different context generations (random, repeats, temporal epsilon greedy)
%- compare performance based on different sizes of context
% sampling methods
% context size

\subsection{Prior Analysis}
In this section we analyse some design choices of the prior.
Some of the results (such as NN architecture) may already be a result of the prior optimization.




==> paper_narrative.tex <==
Paper Narrative Flow 
Title: One-shot World Models Using a Transformer Trained on a Synthetic Prior
(abstract of the abstract of the paper)

Flow Elements: 
    * Purpose - What do you want to explain to the community
        - use purely synthetic random data to pretrain a world model
        - train an agent with few transitions on that trained world model (tbd: how good is the actual agent?) 
        - this world model covers multiple environments without parameter updates
        - (future) planning in world model
    * Executive Summary of the Answer:
        - a purely synthetically pretrained world model can model the dynamics of multiple environments using in-context learning
    * Context - Background, Related Work 
        - Motivation: synthetic data has so far been only used to pretrain / update (world) models but not to getting one-shot world models without weight updates and limited interactions 
        - MBRL / World Models
        - Synthetic Pretraining / PFNs
        - In-context learning / one-shot learning
    * The Method / Solution - How are you approaching the problem
        - Prior Algorithm:
            - 1) sample small random NN for each dimension in state and reward of environment
            - 2) truncate episodes (TODO)
            - 3) 
        - World Model Training Algorithm:
            - 1) initialize world model transformer randomly
            - 2) until done: 
                - 2.1) sample batch consisting of transitions from randomly initialized NNs
                - 2.2) mask transitions at eval pos, have world model transformer predict masked transition
                - 2.3) update world model transformer weights
            - 3) return world model transformer
        - Agent Training Algorithm:
            - 1) load trained world model transformer weights
            - 2) sample 1k transitions context from real environment
            - 3) until agent training done:
                - 3.1) get initial state from real environment
                - 3.2) do RL agent training
            - 4) return trained agent
        
    * Rationale - why
        - see above
    * Limitations 
        - sampling context well is important to get accurate world model dynamics
        - so far works only with fully observable states/environments where the goal is encoded in the dynamics or does not change with each instantiation (e.g. does not work with Four Rooms / Dark Room)
        - computational cost: forward steps of transformer are more expensive than usual MDP steps (at the same time: offers a solution to not having to train a world model and agents are trained efficiently)
        
    * Future Work
        - image observations / very large action/state space dimensionality
        - experiment with done flag
        - encoding goal state to support partially observable environments
        - utilize transformer for planning / MPC
